TORQUE: A Reading Comprehension Dataset of Temporal Ordering Questions

A critical part of reading is being able to understand the temporal relationships between events described in a passage of text, even when those relationships are not explicitly stated. However, current machine reading comprehension benchmarks have practically no questions that test temporal phenomena, so systems trained on these benchmarks have no capacity to answer questions such as "what happened before/after [some event]?" We introduce TORQUE, a new English reading comprehension benchmark built on 3.2k news snippets with 21k human-generated questions querying temporal relationships. Results show that RoBERTa-large achieves an exact-match score of 51% on the test set of TORQUE, about 30% behind human performance.

==> conclusion.tex <==
% !TEX root = root.tex
\section{Conclusion}
\label{sec:conclusion}

Temporal relation extraction has long been an important yet challenging task in natural language processing.
Lack of high-quality data and difficulty in the learning problem defined by previous annotation schemes inhibited performance of neural-based approaches.
The discoveries that LSTMs readily improve the feature-based state-of-the-art CogCompTime on the MATRES and TCR datasets by a large margin not only give the community a strong baseline, but also indicate that the learning problem is probably better defined by MATRES and TCR.
Therefore, we should move along that direction to collect more high-quality data, which can facilitate more advanced learning algorithms in the future.

==> intro.tex <==
%!TEX root = root.tex
\section{Introduction}
\label{sec:intro}
% introduce importance of time, show existing QA systems don't do well on time, show a real example in our data, explain the difference between our annotation scheme and standard QA data (difficulty of querying a graph, our solution, etc.), advantage over temporal relation formalisms, summary of statistics


Time plays a crucial role in understanding events and stories described in natural language text such as news articles, social media, financial reports, and electronic health records.
For instance, \sentence{he won the championship yesterday} is very different from \sentence{he will win the championship tomorrow}: While the first happened in the past and cannot be changed (if we trust the speaker), the second is not guaranteed to happen because we know the speaker is simply making a prediction. 

When there are multiple events, the temporal order among them also matters, altering which may result in different understandings of the same group of events.
For instance, let \event{A}$\to$\event{B} denote that \event{A} is temporally before \event{B}. 
If \sentence{people were angry}$\to$\sentence{police suppressed people}, then it leaves an impression that people got angry and perhaps ended up in violence, and then the police suppressed them to restore order.
Instead, if \sentence{police suppressed people}$\to$\sentence{people were angry}, then it means that people got angry because of the suppression.
The tone of the story is different simply because of a different temporal order.

These relations between an event and a time point (e.g., ``won the championship yesterday'') or between two events (e.g., event \event{A} happened before event \event{B}) are called {\em temporal relations} (\temprelname). We study it in the setup of machine reading comprehension (MRC), i.e., given a piece of text, we ask a computer natural language questions about temporal relations. 

% \begin{table}[h!]
% 	\centering\small
% 	\begin{tabular}{|p{7cm}|}
% 		\hline
% 		\textbf{Example~\addexctr\label{ex:temporal}:}\\
% 		Heavy snow is causing disruption to transport across the UK, with heavy rainfall bringing flooding to the south-west of England. Rescuers searching for a woman trapped in a landslide at her home in Looe, Cornwall, said they had found a body.\\
% 		\hline
% 	\end{tabular}
% \end{table}

\begin{tcolorbox}\small
	\begin{center}
	\textbf{Example~\addexctr\label{ex:mrc on temprel}}
	\end{center}
	\textbf{Passage:} Heavy snow is causing disruption to transport across the UK, with heavy rainfall bringing flooding to the south-west of England. Rescuers searching for a woman trapped in a landslide at her home in Looe, Cornwall, said they had found a body.\\
	\textbf{Example questions:\\}
	\textbf{\tiny What happened before/after/during the snow?}\\
	\textbf{\tiny What happened before/after/when a woman was trapped?}\\
	\textbf{\tiny What happened before/after/when the rescuers found a body?}\\
\end{tcolorbox}

Example~\ref{ex:mrc on temprel} shows an example of MRC on temporal relations.
This problem is interesting and challenging in the following ways. Use example 1 to illustrate these points: what are the events, multiple or no answers, common sense (trapped before died), and reasoning.

Existing works on MRC have studied very little about temporal relations. \missing{a few sentences to overview the presence of time in existing datasets}. As a result, state-of-the-art MRC systems are very brittle when we ask questions like those in Example~\ref{ex:mrc on temprel}. For instance, \missing{...}

To fill in the blank, this paper proposes the first MRC benchmark on temporal relations. Statistics (number of passages, number of questions, number of events, etc.) Quality of annotations. Different domains. Highlight of results.

The rest of this paper is organized as follows.


% When people use natural language to describe and reason about the world, it is assumed that, in most cases, human readers are able to understand these temporal issues, even if the narrative order (i.e., when an event appears in text) is different from the temporal order (i.e., when an event happens in time). However, how to make computers understand semantics related to time has not received enough attention in the NLP community and remains an open challenge.

==> related.tex <==
% !TEX root = root.tex
\section{Related Work}
\label{sec:related}
% In this section, we briefly review the literature of TempRel extraction, especially those that also used neural approaches.

% \vspace{1cm} \qiang{sometimes compile fails because some references are split across pages; use this space to temporally avoid this issue}

%Initiated by \citet{Allen83}, temporal information retrieval has attracted much attention in the past few decades, and an important aspect of it is to extract the TempRels. 
Early computational attempts to TempRel extraction include \citet{MVWLP06,ChambersWaJu07,BethardMaKl07,VerhagenPu08}, which aimed at building classic learning algorithms (e.g., perceptron, SVM, and logistic regression) using {\em hand-engineered features} extracted for each pair of events.
The frontier was later pushed forward through continuous efforts in a series of SemEval workshops \cite{VGSHKP07,VSCP10,ULADVP13,BDSPV15,BSCDPV16,BSPP17}, and significant progresses were made in terms of data annotation \cite{SBFPPG14,CMCB14,MGCAV16,GormanWrPa16}, structured inference \cite{ChambersJu08b,DoLuRo12,CCMB14,NFWR18}, and structured machine learning \cite{YRAM09,LeeuwenbergMo17,NingFeRo17}.

Since TempRel is a specific relation type, it is natural to borrow recent neural relation extraction approaches \cite{ZLLZZ14,ZZHY15,ZhangWa15,XuHuDe16}.
There have indeed been such attempts, e.g., in clinical narratives \cite{DMLBS17,LMDBS17,TFNT17} and in newswire \cite{ChengMi17,MengRu18,LeeuwenbergMo18}.
However, their improvements over feature-based methods were moderate (\citet{LMDBS17} even showed negative results). 
Given the low IAAs in those datasets, it was unclear whether it was simply due to the low data quality or neural methods inherently do not work well for this task.

A recent annotation scheme, \citet{NingWuRo18}, introduced the notion of multi-axis to represent the temporal structure of text, and identified that one of the sources of confusions in human annotation is asking annotators for TempRels across different axes. When annotating only same-axis TempRels, along with some other improvements to the annotation guidelines, MATRES was able to achieve much higher IAAs.\footnote{Between experts: Kohen's $\kappa\approx0.84$. Among crowd workers: accuracy 88\%. More details in \citet{NingWuRo18}.}
This dataset opens up opportunities to study neural methods for this problem.
In Sec.~\ref{sec:system}, we will explain our proposed LSTM system, and also highlight the major differences from previous neural attempts.

% Among those, \citet{DMLBS17}, \citet{LMDBS17}, and \citet{TFNT17} all experimented on clinical narratives, THYME  \cite{SBFPPG14}, and also focused on a specific type of TempRel (i.e., \temprel{contains}). Given the fact that THYME is a very special domain (e.g., \temprel{contains} makes up more than 60\% of its TempRels), we think that it is yet to be seen in other domains.
% \citet{MengRu18} and \citet{LeeuwenbergMo18} are the most recent works to adopt neural methods in the news domain.

==> results.tex <==
% !TEX root = root.tex
\section{Experiments}
\label{sec:experiments}
\subsection{Data}
The MATRES dataset\footnote{\url{http://cogcomp.org/page/publication_view/834}} contains 275 news articles from the TempEval3 workshop \cite{ULADVP13} with newly annotated events and TempRels.
It has 3 sections: TimeBank (TB), AQUAINT (AQ), and Platinum (PT).
We followed the official split (i.e., TB+AQ for training and PT for testing), and further set aside 20\% of the training data as the development set to tune learning rates and epochs.
We also show our performance on another dataset, TCR\footnote{\url{http://cogcomp.org/page/publication_view/835}} \cite{NFWR18}, which contains both temporal and causal relations and we only need the temporal part.
The label set for both datasets are \temprel{before}, \temprel{after}, \temprel{equal}, and \temprel{vague}.
%, and we can see that the label distribution is very similar between the training and test splits.

\begin{table}[htbp!]
\centering\small
\begin{tabular}{c|c|c|c|c}
    \hline
            &	Purpose	&   \#Doc   &   \#Events    &   \#TempRels  \\
    \hline
    TB+AQ   &	Train	&   255     &   8K          &   13K         \\
    PT    	&	Test	&   20      &   537         &   837         \\
    TCR		&	Test	&	25		&	1.3K		&	2.6K		\\
%    \hline
%            &   BEFORE  &   AFTER       &   EQUAL       &   VAGUE       \\
%    \hline
%    TB+AQ   &   50.4\%  &   35.2\%      &   3.3\%       &   11.1\%      \\
%    PT    &   51.0\%  &   32.4\%      &   3.6\%       &   13.0\%      \\
    % Overall &   50.5\%  &   35.0\%      &   3.3\%       &   11.2\%      \\
    \hline
\end{tabular}
\caption{TimeBank (TB), AQUAINT (AQ), and Platinum (PT) are from MATRES \cite{NingWuRo18} and TCR from \citet{NFWR18}.}
\label{tab:stats}
\end{table}

\subsection{Results and Discussion}

We compare with the most recent version of CogCompTime, the state-of-the-art on MATRES.\footnote{\url{http://cogcomp.org/page/publication_view/844}}
Note that in Table~\ref{tab:position}, CogCompTime performed slightly different to \citet{NZFPR18}: CogCompTime reportedly had $F_1$=65.9 (Table~2 Line~3 therein) and here we obtained $F_1$=66.6.
In addition, \citet{NZFPR18} only reported $F_1$ scores, while we also use another two metrics for a more thorough comparison: classification accuracy (acc.) and temporal awareness $F_{\text{aware}}$, where the awareness score is for the graphs represented by a group of related TempRels (more details in the appendix).
%We use three metrics for a more thorough comparison: classification accuracy (acc.), $F_1$, and temporal awareness $F_{\text{aware}}$, where the awareness score is for the graphs represented by a group of related TempRels (more details in the appendix). 
We also report the average of those three metrics in our experiments.

Table~\ref{tab:position} compares the two different ways to handle event positions discussed in Sec.~\ref{subsec:position}: position indicators (P.I.) and simple concatenation (Concat), both of which are followed by network (d) in Fig.~\ref{fig:NN} (i.e., without using Siamese yet).
We extensively studied the usage of various pretrained word embeddings, including conventional embeddings (i.e., the medium versions of word2vec, GloVe, and FastText provided in the Magnitude package \cite{PSCA18}) and contextualized embeddings (i.e., the original ELMo and large uncased BERT, respectively); except for the input embeddings, we kept all other parameters the same.
We used cross-entropy loss and the StepLR optimizer in PyTorch that decays the learning rate by 0.5 every 10 epochs (performance not sensitive to it).

Comparing to the previously used P.I. \cite{DMLBS17}, we find that, with only two exceptions (underlined \qiangchange{in Table~\ref{tab:position}}), the Concat system saw consistent gains under various embeddings and metrics.
In addition, contextualized embeddings (ELMo and BERT) expectedly improved over the conventional ones significantly, although no statistical significance were observed between using ELMo or BERT (more significance tests in Appendix).

\begin{table}[htbp!]
	\centering\small
	\begin{tabular}{ lccccc } 
		\hline
		\textit{System} & \textit{Emb.} & \textit{Acc.} & $F_1$ & $F_{\text{aware}}$	&	Avg.\\
		%\cmidrule(lr){1-2} \cmidrule(lr){3-3} \cmidrule(lr){4-4} \cmidrule(lr){5-5} \cmidrule(lr){6-6} 
		%\multicolumn{2}{l}{CogCompTime} & 61.6 & 66.6 & 60.8 & \textbf{63.0}\\
		\cmidrule(lr){1-6} 
		\multirow{5}{*}{P.I.} 
		& word2vec & 63.2 & 67.6 & \underline{60.5} & 63.8 \\ 
		& GloVe & 64.5 & 69.0 & \underline{61.1} & 64.9\\ 
		& FastText & 60.5 & 64.7 & 59.5 & 61.6\\ \cmidrule(lr){2-6} 
		& ELMo & 67.5 & 73.9 & 63.0 & \textbf{68.1}\\
		& BERT & 68.8 & 73.6 & 61.7 & 68.0\\
		\cmidrule(lr){1-6} 
		\multirow{5}{*}{Concat} 
		& word2vec & 65.0 & 69.5 & 59.4 & 64.6\\ 
		& GloVe & 64.9 & 69.5 & 60.9 & 65.1\\ 
		& FastText & 64.0 & 68.6 & 60.1 & 64.2\\  \cmidrule(lr){2-6} 
		& ELMo & 67.7 & 74.0 & 63.3 & 68.3\\
		& BERT & 69.1 & 74.4 & 63.7 & \textbf{69.1}\\
		\cmidrule(lr){1-6} 
		\multirow{2}{*}{Concat+CSE} 
		& ELMo & 71.7  & 76.7  & 66.0 & \textbf{71.5} \\
		& BERT & 71.3 & 76.3 & 66.5 & 71.4 \\
		\cmidrule(lr){1-6} 
		\multicolumn{2}{l}{CogCompTime\quad\quad\em\em -} & 61.6 & 66.6 & 60.8 & \textbf{63.0}\\
		\hline
	\end{tabular}
	\caption{Performances on the MATRES test set (i.e., \qiangchange{the PT section}). CogCompTime \cite{NZFPR18} is the previous state-of-the-art feature-based system. Position indicator (P.I.) and concatenation (Concat) are two ways to handle event positions in LSTMs (Sec.~\ref{subsec:position}). Concat+CSE achieves significant improvement over CogCompTime on MATRES.}
	\label{tab:position}
\end{table}

\ignore{
\begin{table}[htbp!]
	\centering\small
	\begin{tabular}{ lccccc } 
		\hline
		\textit{System} & \textit{Emb.} & \textit{Acc.} & $F_1$ & $F_{\text{aware}}$	&	Avg.\\
		%\cmidrule(lr){1-2} \cmidrule(lr){3-3} \cmidrule(lr){4-4} \cmidrule(lr){5-5} \cmidrule(lr){6-6} 
		%\multicolumn{2}{l}{CogCompTime} & 61.6 & 66.6 & 60.8 & \textbf{63.0}\\
		\cmidrule(lr){1-6} 
		\multirow{5}{*}{P.I.} 
		& word2vec & 63.2 & 67.6 & \underline{60.5} & 63.8 \\ 
		& GloVe & 64.5 & 69.0 & \underline{61.1} & 64.9\\ 
		& FastText & 60.5 & 64.7 & 59.5 & 61.6\\ \cmidrule(lr){2-6} 
		& ELMo & 67.5 & 73.9 & 63.0 & \textbf{68.1}\\
		& BERT & 68.8 & 73.6 & 61.7 & 68.0\\
		\cmidrule(lr){1-6} 
		\multirow{5}{*}{Concat} 
		& word2vec & 65.0 & 69.5 & 59.4 & 64.6\\ 
		& GloVe & 64.9 & 69.5 & 60.9 & 65.1\\ 
		& FastText & 64.0 & 68.6 & 60.1 & 64.2\\  \cmidrule(lr){2-6} 
		& ELMo & 67.7 & 73.9 & 63.3 & 68.3\\
		& BERT & 69.1 & 74.4 & 63.7 & \textbf{69.1}\\
		\hline
	\end{tabular}
	\caption{Performances on the MATRES test set (i.e., PT). CogCompTime is the previous state-of-the-art, feature-based system. Position indicator (P.I.) and concatenation (Concat) are two ways to handle event positions in LSTMs (Sec.~\ref{subsec:position}).}
	\label{tab:position}
\end{table}
}

Given the above two observations, we further incorporated our common sense encoder (CSE) into ``Concat'' with ELMo and BERT in Table~\ref{tab:position}.
We split \ourkb{} into train (80\%) and validation (20\%). The proposed Siamese network (Fig.~\ref{fig:NN}c) 
% uses dropout of $ 0.3 $ after the embedding layer and first hidden layer \cite{SHKSS14} and 
was trained by minimizing the cross-entropy loss using Adam \cite{KingmaBa14} (learning rate 1e-4, 20 epochs, and batch size 500).  
% The resulting network achieved a mean absolute error (i.e., the average difference between predicted and gold probability) of 0.129 on the validation set, indicating very good generalization to unseen pairs.
%In terms of using the output from the Siamese network, we have two options as explained at the end of Sec.~\ref{subsec:common sense}: (1) to mimic how \citet{NWPR18} used TemProb, i.e., to simply concatenate its output as additional features, and (2) to discretize the output probabilities and use categorical embeddings for each discrete value (the proposed CSE).
We first see that CSE improved on top of Concat for both ELMo and BERT under all metrics,  confirming the benefit of \ourkb{}; second, as compared to CogCompTime, the proposed Concat+CSE achieved about 10\% absolute gains in accuracy and $F_1$, 5\% in awareness score $F_{\text{aware}}$, and 8\% in the three-metric-average metric, with $p<0.001$ per the McNemar's test.  Roughly speaking, the 8\% gain is contributed by LSTMs for 2\%, contextualized embeddings for 4\%, and CSE for 2\%.
Again, no statistical significance were observed between using ELMo and BERT.
%
Table~\ref{tab:cse} furthermore applies CogCompTime and the proposed Concat+CSE system on a different test set called TCR \cite{NFWR18}. Both systems achieved better scores (suggesting that TCR is easier than MATRES), while the proposed system still outperformed CogCompTime by roughly 8\% under the three-metric-average metric, consistent with our improvement on MATRES.
%Lines~4-5 shows the corresponding performance of them on top of the system on Line~3. 
%We can see that they both improved over Line~3, confirming the benefit brought by the external common sense knowledge base; also, Line~5 is showing larger gains, suggesting that CSE is a better option for using it.
%Finally, compared to CogCompTime, the proposed system achieved about 10\% absolute gains in accuracy and $F_1$, and about 5\% in awareness score $F_{\text{aware}}$.

\begin{table}[htbp!]
	\centering\small
	\begin{tabular}{ lccccc } 
		\hline
		\textit{System} & \textit{Emb.} & \textit{Acc.} & $F_1$ & $F_{\text{aware}}$ & Avg.\\
		\cmidrule(lr){1-2} \cmidrule(lr){3-3} \cmidrule(lr){4-4} \cmidrule(lr){5-5} \cmidrule(lr){6-6}
		\multicolumn{2}{l}{CogCompTime~~~~~~-} & 68.1 & 70.7 & 61.6 & \textbf{66.8}\\
		\cmidrule(lr){1-6} 
		%\cmidrule{1-2}
		%		\multirow{2}{*}{4.~3+TemProb} 
		%		& ELMo & 68.7  & 73.9  & 64.9\\
		%		& BERT & 70.3 & 75.2 & 66.1\\
		%		\hline
		\multirow{2}{*}{Concat+CSE} 
		& ELMo & 80.8  & 78.6  & 69.9 & \textbf{76.4} \\
		& BERT & 78.4 & 77.0 & 69.0 & 74.9 \\
		\hline
	\end{tabular}
	\caption{Further evaluation of the proposed system, i.e., Concat (Table~\ref{subsec:position}) plus CSE (Sec.~\ref{subsec:common sense}), on the TCR dataset \cite{NFWR18}.}
	\label{tab:cse}
\end{table}

\ignore{
\begin{table}[htbp!]
	\centering\small
	\begin{tabular}{ lccccc } 
		\hline
		\textit{System} & \textit{Emb.} & \textit{Acc.} & $F_1$ & $F_{\text{aware}}$ & Avg.\\
		\cmidrule(lr){1-2} \cmidrule(lr){3-3} \cmidrule(lr){4-4} \cmidrule(lr){5-5} \cmidrule(lr){6-6} 
		\multicolumn{6}{c}{\underline{\textsc{Test Set: Platinum from MATRES}}}\\
		\multicolumn{2}{l}{CogCompTime} & 61.6 & 66.6 & 60.8 & \textbf{63.0}\\
		%\cmidrule{1-2}
%		\multirow{2}{*}{4.~3+TemProb} 
%		& ELMo & 68.7  & 73.9  & 64.9\\
%		& BERT & 70.3 & 75.2 & 66.1\\
%		\hline
		\multirow{2}{*}{Concat+CSE} 
		& ELMo & 71.7  & 76.7  & 66.0 & \textbf{71.5} \\
		& BERT & 71.3 & 76.3 & 66.5 & 71.4 \\
%		\hline
%		5 vs. 1 & ELMo & +10.1 &+10.1  & +5.2\\
%		5 vs. 1 & BERT & +9.7 & +9.7 & +5.7\\
		\cmidrule{1-6}
		\multicolumn{6}{c}{\underline{\textsc{Test Set: TCR from \citet{NFWR18}}}}\\
		\multicolumn{2}{l}{CogCompTime} & 68.1 & 70.7 & 61.6 & \textbf{66.8}\\
		%\cmidrule{1-2}
		%		\multirow{2}{*}{4.~3+TemProb} 
		%		& ELMo & 68.7  & 73.9  & 64.9\\
		%		& BERT & 70.3 & 75.2 & 66.1\\
		%		\hline
		\multirow{2}{*}{Concat+CSE} 
		& ELMo & 80.8  & 78.6  & 69.9 & \textbf{76.4} \\
		& BERT & 78.4 & 77.0 & 69.0 & 74.9 \\
		\hline
	\end{tabular}
	\caption{The proposed system, i.e., Concat (Sec.~\ref{subsec:position}) plus CSE (Sec.~\ref{subsec:common sense}), achieved significant improvement over CogCompTime, on both MATRES and TCR.}
	\label{tab:cse}
\end{table}
}

% \qiangchange{Note that in our experiments, we used all the embeddings as-is without fine-tuning, so even larger improvements can be expected once fine-tuning is applied.}


==> system.tex <==
% !TEX root = root.tex
\section{Neural TempRel Extraction}
\label{sec:system}

\begin{figure*}[htbp!]
	\centering
	\includegraphics[width=\textwidth]{fig/diagram.pdf}
	\caption{Overview of the neural network structures studied in this paper. Networks (a) and (b) are two ways to handle event positions in LSTMs (Sec.~\ref{subsec:position}). (c) The Siamese network used to fit TemProb (Sec.~\ref{subsec:common sense}). \qiangchange{Once trained on TemProb, the Siamese network is fixed when training other parts of the system.} (d) The FFNN that generates confidence scores for each label. Sizes of hidden layers are already noted. Embeddings of the same color share the same matrix.}
	\label{fig:NN}
\end{figure*}

One major disadvantage of feature-based systems is that errors occurred in feature extraction propagate to subsequent modules.
Here we study the usage of LSTM networks\footnote{We also tried convolutional neural networks but \sanjaychange{did not observe that CNNs improved performance significantly compared to the LSTMs}. Comparison between LSTM and CNN is also not the focus of this paper.} on the TempRel extraction problem as an end-to-end approach that only takes a sequence of word embeddings as input (assuming that the position of events are known).
Conceptually, we need to feed those word embeddings to LSTMs and obtain a vector representation for a particular pair of events,
which is followed by a fully-connected, feed-forward neural network (FFNN) to generate confidence scores for each output label.
Based on the confidence scores, global inference is performed via integer linear programming (ILP), which is a standard procedure used in many existing works to enforce the transitivity property of time \cite{ChambersJu08,DoLuRo12,NingFeRo17}.
An overview of the proposed network structure and corresponding parameters can be found in Fig.~\ref{fig:NN}. Below we also explain the main components.

\subsection{Handling Event Positions}
\label{subsec:position}
Each TempRel is associated with two events, and for the same text, different pairs of events possess different relations, so it is critical to indicate the positions of those events when we train LSTMs for the task.
The most straightforward way is to concatenate the hidden states from both time steps that correspond to the location of those events (Fig.~\ref{fig:NN}b).
\citet{DMLBS17} handled this issue differently, by adding XML tags immediately before and after each event (Fig.~\ref{fig:NN}a).
For example, in the sentence, {\em After \textbf{eating} dinner, he \textbf{slept} comfortably}, where the two events are bold-faced, they will convert the sequence into {\em After $<$e1$>$ eating $<$/e1$>$ dinner, he $<$e2$>$ slept $<$/e2$>$ comfortably.}
The XML markups, which was initially proposed under the name of {\em position indicators} for relation extraction \cite{ZhangWa15}, uniquely indicate the event positions to LSTM, such that the final output of LSTM can be used as a representation of those events and their context.
We compare both methods in this paper, and as we show later, the straightforward concatenation method is already as good as XML tags for this task.

\subsection{Common Sense Encoder (CSE)}
\label{subsec:common sense}
% Common sense has been an essential component for natural language understanding, including temporal relation extraction.
In naturally occurring text that expresses TempRels, connective words such as {\em since}, {\em when}, or {\em until} are often not explicit; nevertheless, humans can still infer the TempRels using common sense with respect to the events. For example, even without context, we know that {\em die} is typically after {\em explode} and {\em schedule} typically before {\em attend}.
\citet{NWPR18} was an initial attempt to acquire such knowledge, by aggregating automatically extracted TempRels from a large corpus. The resulting knowledge base, \ourkb{}, contains observed frequencies of tuples $(v1,v2,r)$ representing the probability of verb 1 and verb 2 having relation $r$ and it was shown a useful resource for TempRel extraction.

However, \ourkb{} is a simple counting model and fails (or is unreliable) for unseen (or rare) tuples.
For example, we may see (ambush, die) less frequently than (attack, die) in a corpus, and the observed frequency of (ambush, die) being \temprel{before} or \temprel{after} is thus less reliable. However, since ``ambush'' is semantically similar to ``attack'', the statistics of (attack, die) can actually serve as an auxiliary signal to (ambush, die).
Motivated by this idea, we introduce common sense encoder (CSE): We fit an updated version of \ourkb{} via a Siamese network \cite{BGLSS94} that generalizes to unseen tuples through the resulting embeddings for each verb (Fig.~\ref{fig:NN}c).
\qiangchange{Note that the \ourkb{} we use is reconstructed using the same method described in \citet{NWPR18} with the base method changed to CogCompTime. Once trained, CSE will remain fixed when training the LSTM part (Fig.~\ref{fig:NN}a or b) and the feedforward neural network part (Fig.~\ref{fig:NN}d). We only use CSE for its output. In the beginning, we tried to directly use the output (i.e., a scalar) and the influence on performance was negligible. 
% It may be because the impact of a single scalar on subsequent networks is, numerically, very limited. 
Therefore, here we discretize the CSE output, change it to categorical embeddings, concatenate them with the LSTM output, and then produce the confidence scores (Fig.~\ref{fig:NN}d).} 
% \footnote{For example, they took the observed frequency of $(e1,e2,r)$ as the estimated probability of event 1 and event 2 being relation $r$, and if such a tuple was not observed, the frequency would be zero.} 
%the other one is that the estimated probabilities of $(v1,v2,r)$ were simply added as extra features to their feature-based system without more advanced neural methods.
%To address it, we introduce common sense encoder (CSE):
%We train a Siamese network to fit TemProb (Fig.~\ref{fig:NN}c), which generalizes to unseen tuples through the resulting embeddings for each verb. We then embed the fitted probabilities into continuous vectors and concatenate them with the output vector of LSTMs, based on which the final output is made (Fig.~\ref{fig:NN}d with option c2). Note that in Fig.~\ref{fig:NN}, we also list option c1 that simply takes the output of network (c) and concatenates it to the two layers in (d); this mimics how \citet{NWPR18} used the statistics in TemProb, and we observe slight performance gain by switching from c1 to c2 in practice.
%\qiang{Maybe drop the comparison between c1 and c2.}
